Deep Learning on Attributed Sequences

Recent research in feature learning has been extended to sequence data, where each instance consists of a sequence of heterogeneous items with a variable length. However, in many real-world applications, the data exists in the form of attributed sequences, which is composed of a set of fixed-size attributes and variable-length sequences with dependencies between them. In the attributed sequence context, feature learning remains challenging due to the dependencies between sequences and their associated attributes. In this dissertation, we focus on analyzing and building deep learning models for four new problems on attributed sequences. Our extensive experiments on real-world datasets demonstrate that the proposed solutions significantly improve the performance of each task over the state-of-the-art methods on attributed sequences.

==> chapters/copyright.tex <==
\newpage
\noindent
\noindent
\begin{center}
{\large \bf Document Confidentiality Statement}
\end{center}

{\normalsize
\noindent \textbf{Copyright} \copyright{} 2017 by Zhongfang Zhuang. 
\\

\noindent All rights reserved. This dissertation proposal is an internal document that contains unpublished material. The information contained in this document is confidential, privileged and only for the information of the intended recipient and may not be used, published or redistributed without the prior written consent of the author. 
}

==> chapters/future.tex <==
\chapter{Future Works}
\label{future}

==> chapters/home.tex <==
\begin{center}
	\textit{I started writing this dissertation in the room I grew up, \\ on the first day in the year of Pig. }
\end{center}

\newpage
